Control from Signal Temporal Logic Specifications with Smooth Cumulative Quantitative Semantics

We present a framework to synthesize control policies for nonlinear dynamical systems from complex temporal constraints specified in a rich temporal logic called Signal Temporal Logic (STL). We propose a novel smooth and differentiable STL quantitative semantics called cumulative robustness, and efficiently compute control policies through a series of smooth optimization problems that are solved using gradient ascent algorithms. Furthermore, we demonstrate how these techniques can be incorporated in a model predictive control framework in order to synthesize control policies over long time horizons. The advantages of combining the cumulative robustness function with smooth optimization methods as well as model predictive control are illustrated in case studies.

==> conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusion}
We introduced a novel smooth quantitative semantics for signal temporal logic, that captures valuable information about system performance. We also presented a smooth model predictive control framework for this semantics.

In the future, we plan to investigate the performance of our methodology on noisy systems from a theoretical point of view. We also aim to extend the notion of cumulative semantics to spatio-temporal logics for multi-agent cooperative control under spatial and temporal constraints.
